MeTTA: Single-View to 3D Textured Mesh Reconstruction with Test-Time Adaptation

Reconstructing 3D from a single view image is a long-standing challenge. One of the popular approaches to tackle this problem is learning-based methods, but dealing with the test cases unfamiliar with training data (Out-of-distribution; OoD) introduces an additional challenge. To adapt for unseen samples in test time, we propose MeTTA, a test-time adaptation (TTA) exploiting generative prior. We design joint optimization of 3D geometry, appearance, and pose to handle OoD cases with only a single view image. However, the alignment between the reference image and the 3D shape via the estimated viewpoint could be erroneous, which leads to ambiguity. To address this ambiguity, we carefully design learnable virtual cameras and their self-calibration. In our experiments, we demonstrate that MeTTA effectively deals with OoD scenarios at failure cases of existing learning-based 3D reconstruction models and enables obtaining a realistic appearance with physically based rendering (PBR) textures.

==> figures/tex/abla.tex <==
\begin{wrapfigure}{r}{0.49\linewidth}
  \small
  \centering
    \vspace{-5mm}
    \includegraphics[width=0.99\linewidth]{figures/abla.pdf}
    \vspace{0.1mm}
    \caption{\textbf{Ablation studies.} 
    To validate our pipeline design, we perform ablation studies where the prediction of the initial mesh or initial viewpoint is absent.
    In the case of a missing initial mesh, we initialize our 3D space with ellipsoid.
    Canonical viewpoint means that the azimuth and elevation angles are 0$^\circ$.
    }
    \vspace{-5mm}
  \label{fig:abla}
\end{wrapfigure}

==> figures/tex/counterpart_diffusion.tex <==
\begin{wrapfigure}{r}{0.6\linewidth}
  \small
  \centering
    \includegraphics[width=0.99\linewidth]{figures/counterpart_diffusion.pdf}\vspace{2mm}
    \caption{\textbf{Comparison with 2D generative prior methods.} 
    We compare the single image to 3D reconstruction capability about 2D generative prior methods with the latest work~\cite{melas2023realfusion, tang2023makeit3d}.
    }
  \label{fig:count_diff}
\end{wrapfigure}

==> figures/tex/counterpart_tta.tex <==
\begin{wrapfigure}{r}{0.5\linewidth}
  \small
  \centering
    \includegraphics[width=0.99\linewidth]{figures/counterpart_tta.pdf}
    \caption{\textbf{Comparison with the single-view 3D mesh methods on the in-domain setting (Pix3D).} 
    We compare the single image to 3D reconstruction capability about feed-forward methods~\cite{total3d, zhang2021holisticim3d}.
    Our method shows impressive quality improvement in geometry and also reconstructs realistic texture.
    }
  \label{fig:count_tta}
\end{wrapfigure}

==> figures/tex/domain_gap.tex <==
\begin{wrapfigure}{r}{0.49\linewidth}
  \small
  \centering
    % \vspace{-5mm}
    \includegraphics[width=0.99\linewidth]{figures/domain_gap.pdf}
    \vspace{1mm}
    \caption{\textbf{Distribution gap between train and test.}
    [Left] Input reference images. 
    [Middle] Predicted meshes obtained from the existing feed-forward method~\cite{zhang2021holisticim3d}.
    % It shows that the resulting mesh of the sample from the training domain complies plausibly with the input object, while the mesh generated from the test sample seems to be restricted within a  different shape space.
    [Right] The reconstruction results of $\ours$. 
    Here, ``Train'' refers to a sample on which the Image-to-3D shape method is trained, 
    and ``Test'' is an in-the-wild sample we captured.
    % and ``Test'' is a sample acquired by ourselves.
    % Ours shows high-fidelity geometry and textures even with OoD samples.
     }
     \vspace{-4mm}
  \label{fig:domain_gap}
\end{wrapfigure}

==> figures/tex/pbr.tex <==
\begin{wrapfigure}{r}{0.49\linewidth}
  \small
  \centering
    \vspace{-5.4mm}
    \includegraphics[width=0.99\linewidth]{figures/pbr.pdf}
    \vspace{0.1mm}
    \caption{\textbf{Practical applications in graphics.}
    % With an optimized PBR texture map, we can conduct test-time relighting and material editing with optimized textured mesh in a real graphics engine.
    [PBR Recon.] means reconstruction results with PBR textures by ours.
    }
    \vspace{-4mm}
  \label{fig:pbr}
\end{wrapfigure}

==> figures/tex/qual_ours.tex <==
\begin{figure*}[h]
  \small
  \centering
    \includegraphics[width=0.9\linewidth]{figures/ours.pdf}
    \vspace{2mm}
    \caption{\textbf{Qualitative results of $\ours$ on the in-domain setting (Pix3D).}
    [Input Image] is the reference single-view image given at test time.
    [Initial Mesh] is the initial mesh prediction from the feed-forward mesh prediction stage.
    [Input View.] is the reconstruction results from the input viewpoint, which shows a well-aligned 2D image and our 3D space with the virtual camera.
    [Novel Views] are the reconstructed textured mesh results with novel views (\ie, unseen views).
    \ours~shows impressive fine-grained detailed geometry and realistic textures.
    Even with the backward view of the chair in the first row, ours can reconstruct the complete front view.
    We validate these results with Pix3D dataset~\cite{sun2018pix3d}.
    }
  \label{fig:qual_ours}
\end{figure*}


==> figures/tex/real.tex <==
\begin{figure}[t]
  % \small
  \centering
    \includegraphics[width=0.93\linewidth]{figures/real.pdf}
    \caption{\textbf{Unseen real-world experiments.} 
    We showcase the effectiveness of our test-time adaptation about manually acquired data in real-world scenarios.
    }
  \label{fig:real}
  % \centering
  %   \includegraphics[width=0.93\linewidth]{figures/3dfront.pdf}
  %   \caption{\textbf{Unseen cross-domain experiments about 3D-Front~\cite{fu20213dfront}.} 
  %   We showcase the effectiveness of our test-time adaptation in cross-domain scenarios.
  %   }
% \end{figure*}
\end{figure}

==> figures/tex/virtual_camera.tex <==
\begin{wrapfigure}{r}{0.45\linewidth}
  \small
  \vspace{-4mm}
  \centering
    \includegraphics[width=0.99\linewidth]{figures/view.pdf}
    \vspace{0.1mm}
    \caption{\textbf{Virtual camera.} 
    We represent $\theta, \phi$, and $r$ for elevation angle, azimuth angle, and radius.
    The input image is taken with viewpoint (\clovagreen{$\theta_{ref}, \phi_{ref}, r_{ref}$}), which we estimate and optimize.
    \textbf{\clovagreen{Green dot}} means predicted viewpoint given single-view image.
    \textbf{\royalblue{Blue dot}} means canonical viewpoint with both elevation and azimuth angles are 0$^{\circ}$.
    % If one image is given with viewpoint ($\theta_{ref}, \phi_{ref}, r_{ref}$), and we want to generate another view with viewpoint ($\theta_{new}, \phi_{new}, r_{new}$).
    % It can be conducted by sampling
    % ($\theta_{new} - \theta_{ref}, \phi_{new} - \phi_{ref}, r_{new} - r_{ref}$) as a condition to the multi-view diffusion models, equivalent to the relative viewpoint ($\Delta\theta, \Delta\phi, \Delta r$).
    }
    \vspace{-4mm}
  \label{fig:view}
\end{wrapfigure}

==> supp_fig/tex/pbr.tex <==
\begin{figure}[h]
  \small
  \centering
    \includegraphics[width=0.9\linewidth]{supp_fig/pbr.pdf}
    \caption{\textbf{Limitation of transparency or reflection surface.} 
    The surface texture of the input image is transparent and features special material properties of the mesh.
    As a result, both the output geometry and texture are degraded.
    }
  \label{fig:supp_pbr}
\end{figure}

==> supp_fig/tex/radius_abla.tex <==
\begin{figure}[h]
  \small
  \centering
    \includegraphics[width=0.9\linewidth]{supp_fig/radius_abla.pdf}
    \caption{\textbf{The necessity of learnable virtual camera.} 
    Using an inappropriate radius in the virtual camera space can lead to issues such as exceeding the camera space boundaries, as seen in the green box, or causing degradation of details.
    }
  \label{fig:supp_radius}
\end{figure}

==> supp_fig/tex/segment.tex <==
\begin{figure}[t]
  \small
  \centering
    \includegraphics[width=\linewidth]{supp_fig/segment.pdf}
    \caption{\textbf{Limitation of model dependencies.} 
    The green square indicates object occlusion in the input image, which disrupts segmentation, leading to the disappearance of the reconstruction mesh.
    }
  \label{fig:supp_segment}
\end{figure}

==> tables/compute_time.tex <==
\begin{wrapfigure}{r}{0.5\linewidth}
    \centering
    \small
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l c}
        \toprule
            Method & Optimization Time (min.) \\
         \midrule
             RealFusion~\cite{melas2023realfusion} & 193 \\
             Zero-1-to-3~\cite{liu2023zero123} & - \\
             Make-It-3D~\cite{tang2023makeit3d} & 91 \\
             $\ours$ (ours) & 30 \\
         \bottomrule
    \end{tabular}
    }\vspace{3mm}
    \caption{\textbf{Comparisons of training time.}
    We compare training time between the latest 
    2D generative prior methods \cite{melas2023realfusion, tang2023makeit3d} and $\ours$.
    Other methods need multiple training stages, \eg, textual inversion~\citep{gal2022textualinversion}, so they take significant time to optimize.
    }
    \label{tab:compute_time}
\end{wrapfigure}



==> tables/quan_geo.tex <==
\begin{table}
    \centering
    \small
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{c cccc}
        \toprule
            Metric &  MGN~\cite{total3d} & LIEN~\cite{zhang2021holisticim3d} & \ours~(Ours) \\
        \midrule
            Chamfer Distance $\downarrow$   & 0.1019 & 0.0895 & \textbf{0.0867} \\
        \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Cross-domain evaluation of the single-view to mesh reconstruction.} 
    We measure Chamfer Distance between point clouds uniformly sampled from the predicted and ground-truth mesh. 
    Point clouds are normalized in scale and aligned to the ground-truth point clouds by the iterative closest point (ICP) algorithm. 
    10K points are sampled for each mesh.
    We conduct the experiment to show the test-time adaptation ability of unseen test dataset, 3D-Front~\cite{fu20213dfront}.
    }
    \label{tab:quan_geo}
\end{table}

==> tables/quan_tex.tex <==
\begin{table*}
    \centering
    \small
    \begin{tabular}{l  ccc  cc}
    \toprule
        \multirow{2}[2]{*}{Method} & \multicolumn{3}{c}{Reference View} & \multicolumn{2}{c}{Novel Views} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-6}
        & LPIPS $\downarrow$ & PSNR [dB] $\uparrow$ & CLIP Score $\uparrow$ &  CLIP Score $\uparrow$ & min. CLIP Score $\uparrow$\\ 
    \midrule
        RealFusion~\cite{melas2023realfusion}   & 0.1809 & 21.56 & 0.8494 & 0.7538 & 0.7030 \\
        Make-It-3D~\cite{tang2023makeit3d}   & 0.0867 & 22.45 & 0.9386 & 0.8937 & 0.8046 \\
        $\ours$ (ours)       & \textbf{0.0777} &  \textbf{22.89} & \textbf{0.9465} & \textbf{0.8942} & \textbf{0.8286} \\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{\textbf{Comparisons of texture reconstruction and perceptual quality.}
    We measure the LPIPS,
    PSNR, and CLIP Score at the reference view and novel views.
    For the comparison of novel view renderings, we render the same number and location of viewpoints for all methods.
    }
    \label{tab:quan_tex}
\end{table*}
